UNO Push: Unified Nonprehensile Object Pushing via Non-Parametric Estimation and Model Predictive Control

Nonprehensile manipulation through precise pushing is an essential skill that has been commonly challenged by perception and physical uncertainties, such as those associated with contacts, object geometries, and physical properties. For this, we propose a unified framework that jointly addresses system modeling, action generation, and control. While most existing approaches either heavily rely on a priori system information for analytic modeling, or leverage a large dataset to learn dynamic models, our framework approximates a system transition function via non-parametric learning only using a small number of exploratory actions (ca. 10). The approximated function is then integrated with model predictive control to provide precise pushing manipulation. Furthermore, we show that the approximated system transition functions can be robustly transferred across novel objects while being online updated to continuously improve the manipulation accuracy. Through extensive experiments on a real robot platform with a set of novel objects and comparing against a state-of-the-art baseline, we show that the proposed unified framework is a light-weight and highly effective approach to enable precise pushing manipulation all by itself. Our evaluation results illustrate that the system can robustly ensure millimeter-level precision and can straightforwardly work on any novel object.

==> includes/implementation.tex <==
\section{Implementation}


To apply the control methods above into the practical planar pushing task, a scheme is needed for the robot to perform a smooth and adjustable push with the generated action. 

In each iteration of the loop, the end-effector will firstly move to the Pre-push point mentioned in Section III , denoted as $\hat{X}_{robot}^{start}$, then performs the push action using the current control input $u_t$ and obtains the object state after the push ${X}_{t+1}$ to calculate the change of the state ${X}_{t+1}^t$.

Next, the algorithm updates the GP model by calling the function $Refine({u_t,X_{t+1}^t}, \hat{\Gamma}_t)$ using the current control input and the new object state to refine the model, as mentioned in Section IV. We then calculates the next control input $u_{t+1}$ using the function $GetAct(X_{obj},X_{Target},\hat{\Gamma}_{t+1})$ where the control methods in Section V take part in.

One of the critical aspects of our scheme is the action switching process, which is essential for smooth and efficient nonprehensile manipulation. The goal is to enable the robot to move continuously during the transition between actions to push the object smoothly and reduce the number of pushes required. However, this may cause unexpected displacement of the object, particularly when the pushing direction between two actions differs significantly.

To address this problem, we compare the control input $u_{t+1}$ of the new action with the current control input $u_t$. If the change in control input is less than a predefined threshold $\Delta a$, the algorithm switches to the new action continuously by calling the $SwitchPush(u_t,u_{t+1})$ function to perform a smooth transition. Otherwise, the robot will retreat to the previous starting state and move to the new starting state for a new iteration of the loop. Although the threshold for the difference between actions cannot be precisely estimated due to the unknown object shape, we can still improve the efficiency while tolerating some loss in accuracy, which can be corrected using a close-loop control method.







\begin{algorithm}
\caption{Pushing scheme}
\algtext*{EndIf}% Remove "end if" text
\algtext*{EndFor}% Remove "end for" text
\begin{algorithmic}[1]
\State Initialization: $X_{robot}$, $X_{0}$, $u_0$, $\hat{\Gamma}_0$, $t=0$

\State  $\hat{X}_{robot}^{start}$ $\gets$ Start($u_t$, $X_t$)
\While {Goal is met}
\State  $\hat{X}_{robot}^{push}$ $\gets$ Push($u_t$)\Comment{perform the push}
\State $X_{t+1}^t \gets X_{t+1}\cdot X_t^{-1}$ \Comment{sensor}
\State  $\hat{\Gamma}_{t+1} \gets$ Refine$(\{u_t, X_{t+1}^t\}, \hat{\Gamma}_t)$\Comment{(12)}

\State $u_{t+1}$ $\gets$ GetAct($X_{obj}$, $X_{Target}$, $\hat{\Gamma}_{t+1}$)
\If{Evaluate($u_t$, $u_{t+1}$)$<\Delta a$}\Comment{switch action}
\State  $\hat{X}_{robot}^{switch}$ $\gets$ SwitchPush($u_t$, $u_{t+1}$)

\Else \Comment{restart}\State $\hat{X}_{robot}^{retreat}\gets$ Retreat($X_{t+1}$) 

\State  $\hat{X}_{robot}^{start}$ $\gets$ Start($u_{t+1}$, $X_{t+1}$)
\EndIf
\State $t\gets t+1$

\EndWhile
\end{algorithmic}
\end{algorithm}
